An Efficient Algorithm for Power Dominating Set

The problem Power Dominating Set (PDS) is motivated by the placement of phasor measurement units to monitor electrical networks. It asks for a minimum set of vertices in a graph that observes all remaining vertices by exhaustively applying two observation rules. Our contribution is twofold. First, we determine the parameterized complexity of PDS by proving it is $W[P]$-complete when parameterized with respect to the solution size. We note that it was only known to be $W[2]$-hard before. Our second and main contribution is a new algorithm for PDS that efficiently solves practical instances. Our algorithm consists of two complementary parts. The first is a set of reduction rules for PDS that can also be used in conjunction with previously existing algorithms. The second is an algorithm for solving the remaining kernel based on the implicit hitting set approach. Our evaluation on a set of power grid instances from the literature shows that our solver outperforms previous state-of-the-art solvers for PDS by more than one order of magnitude on average. Furthermore, our algorithm can solve previously unsolved instances of continental scale within a few minutes.

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

The goal of this section is threefold.
First, we evaluate the performance of our algorithm in comparison to two previous state-of-the-art approaches.
Secondly, we give a more detailed view on the performance by analyzing how the upper and lower bounds found be the different algorithms converge to the optimal solution.
Thirdly, we evaluate the impact of the different reduction rules.

\subparagraph{Experiment Setup.}

We implemented our algorithm in C++ 20 and compiled it with clang 15.0.1 with the \texttt{-O3} optimization flag.
Our source code along with all data sets and evaluation scripts is available on GitLab\footnote{\url{https://gitlab.com/Aldorn/pds-code}}.
For the comparison with the previous state-of-the-art, we use the MILP formulation approach by Jovanovic and Voss \cite{jovanovic2020fixed}.
In the following, we refer to this algorithm with \texttt{MILP}.
The second solver by Smith and Hicks~\cite{smith2020OptimalSP} and is based on the implicit hitting set approach.
Unfortunately, their code is not publicly available, and the paper does not specify all implementation details.
To make a fair (or rather generous) comparison, we initialized their set of forts with our fort heuristic, which, as far as we can judge, leads to better results than reported in the original publication~\cite{smith2020OptimalSP}.
We refer to this algorithm as \texttt{MFN} (abbreviation for \emph{minimum fort neighborhood}).
For the implicit hitting set approaches, we use an MILP formulation to solve the \HS instances.
All MILP instances are solved using Gurobi~9.5.2~\cite{gurobi}.

The experiments were run on a machine running Ubuntu 22.04 with Linux 5.15.
The machine has two Intel\textregistered Xeon\textregistered Gold 6144 CPUs clocked at 3.5 GHz with 8 single-thread cores and 192 GB of RAM.

We used a collection of instances shipped with pandapower~\cite{thurner2018pandapower}.
We further use the Eastern, Western, Texas and US instances from the powersimdata set\footnote{\url{https://github.com/Breakthrough-Energy/PowerSimData}}~\cite{Xu2020powersimdata} based on the US electric grids.
We interpret the power grids as graphs were buses are vertices and power lines and transformers are edges.
Buses without attached loads or generators yield propagating vertices.
For experiments on the pandapower instances, we used a timeout of \SI{2}{h} and repeated each experiment 5 times.
On the powersimdata instances, we used a timeout of \SI{10}{h} and only repeated the experiments using our solver.
For repeated experiments, we report the median result.

\subparagraph{Performance Comparison.}

We compare the performance of our solver to the \texttt{MILP} and \texttt{MFN} approach, each with and without preprocessing by the reduction rules.
To assess the performance of our approach with reduction rules, we compute the speedup compared to the lowest run time of the previous approaches without reduction rules.

\begin{table}
\caption{Run times of different combinations of \Pds solvers and reduction rules on the pandapower data set. Note that $\gamma_P$ differs from the results reported in other literature. This is to be expected because we include non-propagating vertices from the input. Further observe that some run times are given in milli- or microseconds.}
\label{tbl:solver comparison normal}
%\hspace{-1.5cm}
\footnotesize
  \begin{threeparttable}
\pgfplotstabletypeset[
  string type,
  columns={name,pmus,jovanovic,jovanovic-r,bozeman-smith,bozeman-smith-r,ours,ours-r,speedup},
  columns/name/.style={
    column type=l,
    column name=instance,
    string type,postproc cell content/.append style={/pgfplots/table/@cell content/.add={\ttfamily}{}}
  },
  columns/pmus/.style={column name={$\gamma_P$}},
  columns/bozeman-smith/.style={column name={\texttt{MFN}\tnote{a}}},
  columns/bozeman-smith-r/.style={column name={\texttt{MFN+R}\tnote{a}}},
  columns/jovanovic/.style={column name={\texttt{MILP}\tnote{a}}},
  columns/jovanovic-r/.style={column name={\texttt{MILP+R}\tnote{a}}},
  columns/ours/.style={column name={Ours}},
  columns/ours-r/.style={column name={Ours+R}},
  columns/speedup/.style={column name={Speedup\tnote{b}},numeric type,fixed, fixed zerofill,precision=1},
  every head row/.style={
    before row=\toprule,
    after row={\texttt{case*}&\multicolumn{1}{c}{\#}&\multicolumn{1}{c}{s}&\multicolumn{1}{c}{s}&\multicolumn{1}{c}{s}&\multicolumn{1}{c}{s}&\multicolumn{1}{c}{s}&\multicolumn{1}{c}{s}\\\midrule},
  },
  every last row/.style={
    after row=\bottomrule,
  },
  every even row/.style={before row={\rowcolor[gray]{0.9}}},
  column type=r,multicolumn names,
]{tables/solver-times.csv}
\begin{tablenotes}
  \item[a] numbers here were obtained from our interpretation of the respective approach
  \item[b] speedup of Ours+R compared to the faster of \texttt{MILP} and \texttt{MFN}
  \item[c] solved optimally by reduction rules
\end{tablenotes}
\end{threeparttable}
\end{table}

\Cref{tbl:solver comparison normal} shows the run times of the solvers on the smaller pandapower instances.
Preprocessing significantly reduced the running times of all solvers in most cases, especially for the larger instances.
In fact, we found that our reduction rules were able to solve 9 out of 26 instances on their own.
In those cases, no solver without reduction rules could compete.
Out of the remaining instances, our our solver without reduction rules was the fastest on 3 instances while our solver with reduction rules was the fastest on all others.

For the larger powersimdata instances, neither \texttt{MILP} nor \texttt{MFN} were able to compute an optimal solution without using our reduction rules within the time limit.
Thus, for these instances, we only compare our solver with \texttt{MFN+R} and \texttt{MILP+R}.
Table~\ref{tbl:solver comparison large} shows the results.
Observe that for \texttt{Eastern}, our algorithm finished after \SI{16}{min} while \texttt{MFN} did not finish after more than \SI{6}{h}, with a lower bound that was still more than 100 vertices below the optimal solution.
Observe that the number of fort neighborhoods $|\mathcal F|$ is slightly lower for \texttt{MFN}, which is to be expected as this is basically the main goal of \texttt{MFN} when finding new fort neighborhoods.
However, this clearly does not show any benefit in the resulting run time.

\begin{table}
  \caption{Run times of different combinations of \Pds solvers and reduction rules on the pandapower data set with all vertices considered propagating. Observe that some run times are given in milli- or microseconds.}
%  \caption{Median running times of different combinations of \Pds solvers and reduction rules on the instance with only propagating vertices.}
  \label{tbl:solver comparison all propagating}
%  \hspace{-1.5cm}
\footnotesize
  \begin{threeparttable}
    \pgfplotstabletypeset[
    ignore chars={"},
    string type,
  columns={name,pmus,jovanovic,jovanovic-r,bozeman-smith,bozeman-smith-r,ours,ours-r,speedup},
    columns/name/.style={
      column type=l,
      column name=instance,
      string type,postproc cell content/.append style={/pgfplots/table/@cell content/.add={\ttfamily}{}}
    },
    columns/pmus/.style={column name={$\gamma_P$}},
    columns/bozeman-smith/.style={column name={\texttt{MFN}\tnote{a}}},
    columns/bozeman-smith-r/.style={column name={\texttt{MFN+R}\tnote{a}}},
    columns/jovanovic/.style={column name={\texttt{MILP}\tnote{a}}},
    columns/jovanovic-r/.style={column name={\texttt{MILP+R}\tnote{a}}},
    columns/ours/.style={column name={Ours}},
    columns/ours-r/.style={column name={Ours+R}},
    columns/speedup/.style={column name={{Speedup}\tnote{b}},numeric type,fixed, fixed zerofill,precision=1},
    every head row/.style={
      before row=\toprule,
      after row={\texttt{case*}&\multicolumn{1}{c}{\#}&\multicolumn{1}{c}{s}&\multicolumn{1}{c}{s}&\multicolumn{1}{c}{s}&\multicolumn{1}{c}{s}&\multicolumn{1}{c}{s}&\multicolumn{1}{c}{s}\\\midrule},
    },
    every last row/.style={
      after row=\bottomrule,
    },
    every even row/.style={before row={\rowcolor[gray]{0.9}}},
    column type=r,multicolumn names,
    ]{tables/solver-times-z.csv}
    \begin{tablenotes}
      \item[a] numbers here were obtained from our interpretation of the respective approach
      \item[b] speedup of Ours+R compared to the faster of \texttt{MILP} and \texttt{MFN}
      \item[c] solved optimally by reduction rules
    \end{tablenotes}
  \end{threeparttable}
\end{table}

In the literature, most other solvers only consider networks consisting solely of propagating vertices.
For comparison, we conducted the experiment on the same instances but with all vertices propagating, see \cref{tbl:solver comparison all propagating}.
Observe that $\gamma_P$ is lower when all vertices are propagating.
With only propagating vertices in the input, our reduction rules could solve 13 out of 26 instances on their own.
On all remaining instances, our solver combined with the reduction rules was the fastest and achieved a median speedup of 176.2.

Comparing the results in \cref{tbl:solver comparison all propagating} and \cref{tbl:solver comparison normal}, we observe that the solvers react differently to all vertices being propagating.
While \texttt{MILP} and our solver without reductions are somewhat faster with some non-propagating vertices in the input, \texttt{MFN} and our solver with reductions perform better when all vertices are propagating.
This leads to an interesting effect: Overall, \texttt{MILP} performs better than \texttt{MFN} when the input contains non-propagating vertices but considerably  worse when all vertices are propagating.
Nonetheless, our solver remains the fastest in both cases.


%We obtained similar results when considering all vertices in the instances propagating.
%This is the version of the problem commonly discussed in the literature.
%With these instances as inputs, our solver was the fastest on 16 out of 26 instances.\todo{update numbers}
%We achieved a median speedup of around 52.9.
%The median speedup over all instances with only propagating vertices was 449, with higher speedups in larger instances.

\begin{table}
  \footnotesize
  \caption{
    Comparison between our algorithm, \texttt{MILP} and \texttt{MFN} on the larger powersimdata US instances preprocessed with our reduction rules.
    The number of vertices is $n$, $|Z|$ is the number of non-propagating vertices and $\abs{\mathcal F}$ is the size of the arising hitting set instance, if applicable.
    For the solvers, we report the power dominating number $\gamma_P$ (or the best found lower bound) as well as the number of fort neighborhoods $\mathcal F$ and the run time.
  }
  \label{tbl:solver comparison large}
  \begin{tabular}{l r r r r r r r r r r}
    \toprule
  & \multicolumn{2}{c}{Input} & \multicolumn{3}{c}{Our  Solver} & \multicolumn{3}{c}{\texttt{MFN+R}} & \multicolumn{2}{c}{\texttt{MILP+R}} \\\cmidrule(rl){2-3}\cmidrule(rl){4-6}\cmidrule(rl){7-9}\cmidrule(rl){10-11}
  Instance                             & $n$   & $\abs{Z}$ & $\gamma_P$ & $\abs{\mathcal{F}}$ & $t$~(s) & $\gamma_P$ & $\abs{\mathcal{F}}$ & $t$~(s) & $\gamma_P$ & $t$~(s) \\\midrule
  \rowcolor[gray]{0.9}\texttt{Texas}   & 2000  & 376   & 411   & 838   & 0.98   & 411    & 659     & 17.73        & 411    & 1.81 \\
  \texttt{Western}                     & 10024 & 4106  & 1825  & 2618  & 1.55   & 1825   & 2010    & 158.51       & 1825   & 2.16 \\
  \rowcolor[gray]{0.9}\texttt{Eastern} & 70047 & 30332 & 12895 & 27019 & 552.46 & >12789 & >15043  & >\SI{10}{h}  & >12890 & >\SI{10}{h} \\
  \texttt{USA}                         & 82071 & 34814 & 15131 & 30357 & 728.62 & >14124 & >16391  & >\SI{10}{h}  & >15126 & >\SI{10}{h} \\\bottomrule
  \end{tabular}
\end{table}

\subparagraph{Lower and Upper Bounds.}

We note that all three approaches find lower bounds while solving the instances.
In case of the implicit hitting set approeach, each time we solve the current \HS instance, the solution size is a lower bound for a minimum power dominating set.
This yields lower bounds for our approach as well as for \texttt{MFN}.
Moreover, Gurobi also provides lower bounds for \texttt{MILP}.
Additionally, Gurobi provides upper bounds.
To also get upper bounds for the implicit hitting set approaches, we use the following greedy heuristic.
Whenever we have computed a hitting set $H$ of the current fort neighborhoods, we greedily add vertices to $H$, preferably selecting vertices with many unobserved neighbors, until we have a power dominating set.
Afterwards, we make sure that the resulting solution is minimal with respect to inclusion.

With this, we can observe how quickly the different algorithms converge towards the optimal solution.
\Cref{fig:exp:bounds and gap} illustrates the behavior of the bounds with respect to the time for two of the four powersimdata instances.
All three algorithms use our reduction rules (recall that neither \texttt{MILP} nor \texttt{MFN} were able to solve these instances without them).
We clearly see that, with our approach, the gap between upper and lower bounds shrinks quickly, in particular compared to \texttt{MFN}.
This validates our assumption that adding many -- potentially larger -- forts instead of a single minimum size one is highly beneficial.
Recall that \texttt{MFN} can increase its lower bound only by at most $1$ after finding a new hitting set while we can increase the lower by up to one for each undecided unhit vertex.

Interestingly, for \texttt{MILP+R} the gap between upper and lower bound closes much quicker than for \texttt{MFN+R}.
In particular, for the largest \texttt{USA} instance, there is almost no gap left after little more than \SI{100}{s}.
Gurobi also found an optimal solution, but failed to prove the lower bound on its size within the timeout of \SI{10}{h}.
Thus, in cases where a good approximation is acceptable, the \texttt{MILP} formulation (with our reduction rules) is not much worse than our approach.

\begin{figure}
  \begin{center}
    \input{figures/evaluation/bounds_gap.tikz}
  \end{center}
  \vspace{-1\baselineskip}
  \caption{Upper and lower bounds on the optimum value on the \texttt{Texas} and \texttt{USA} powersimdata instances with preprocessing by our reduction rules. We give the bounds reported by our solver and by \texttt{MFN}, both with added greedy upper bounds, as well as Gurobi for \texttt{MILP}. Note that the x axis uses a logarithmic scale.}
  \label{fig:exp:bounds and gap}
\end{figure}

\subparagraph{Reduction Rules.}

\begin{figure}
  \centering
  \input{figures/evaluation/running_times.tikz}
  \vspace{-2\baselineskip}

  \subcaptionbox{Median running time on each instance with the different subsets of reduction rules\label{fig:exp:reduction running times}}[.48\linewidth]{~}\hfill
  \subcaptionbox{Aggregated speed-up of each set of reduction rules compared to our algorithm without reduction rules\label{fig:exp:reduction speed up}}[.48\linewidth]{~}

  \caption{Running times  and speed-up of our algorithm with different subsets of the reduction rules on the pandapower instances.}
  \label{fig:exp:running time and sped up}
\end{figure}

To evaluate the effect of the reduction rules on the performance of our algorithm, we let it run on the pandapower instances with different subsets of reduction rules.
Recall that we have several local reduction rules as well was the two non-local rules \ref{red:domination} and \ref{red:necessary}.
In addition to using all or no reduction rules, we consider the following subsets.
Only local rules, only non-local rules, all local rules together with \ref{red:domination}, and all local rules together with \ref{red:necessary}.

\Cref{fig:exp:reduction running times} shows the median running time for each instance in the different settings.
In most instances, the reductions could decrease the running time by an order of magnitude or more.
Moreover, we can see that in most cases all reduction rules are relevant, i.e., we achieve the lowest run time when using all reduction rules and applying no reduction rules is usually slower than applying any of the rules.

\Cref{fig:exp:reduction speed up} shows the speedup aggregated over all instances of using reduction rules compared to using no reduction rules for our solver.
We can see that the median speedup is roughly one order of magnitude when applying all reduction rules.
The most interesting observation here is that local+\ref{red:necessary} does not give any improvement compared to just local.
In fact, it is slightly slower.
However, when combined with \ref{red:domination}, \ref{red:necessary} gives a significant improvement.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> figures/booster/short.tex <==
\tikzpicturename{booster-short}
\tikz[pds instance] \graph[nodes={node,propagating},empty nodes] {a["$x$"] -- b[booster] -- c["$y$"]};


==> figures/implication/short.tex <==
\tikzpicturename{gadget-implication-short}
\begin{tikzpicture}[baseline={(a.south)},pds instance]
	\graph[empty nodes,grow right=2] {[nodes={node,propagating}] a["$x$"] -> b["$y$"]};
\end{tikzpicture}


==> sections/variants.tex <==
\section{Power Dominating Set-Variants}
\label{sec:variants}

\todoin{Abschnitt vollständig überarbeiten, Verschieben in Conclusion?}

Different authors have studied both restricted and extended versions of \PDS.
In case of \DS the \textsc{Connected \DS} problem is of greater interest.
It asks for a dominating set $S$ of $G$ that induces a connected subgraph in $G$.
This can be easily extended to \textsc{Connected \PDS}: Does $G$ have a connected power dominating set of size at most $k$?
This version of \Pds is also \W{P} complete.
The reduction to show \W{P}-hardness is essentially the same as above, but with additional edges between the booster node $b$ and the nodes in the input clique $X$.
This allows the input vertices and $b$ to observe one another but this not allow the propagation rule to be applied to vertices to which it could not be applied before.
Using \cref{thm:wp contained ntm} we can see that it is also in \W{P}.

Another natural extension is $l$-\PDS($l$-\Pds) where the propagation rule is modified, such that a vertex observes its neighborhood if it is observed and has at most $l$ unobserved neighbors.
In other works this variant is usually called \Pds[k], but we use $k$ as parameter for the size of the power dominating set.
This generalization includes both \DS as \Pds[0] and classical \Pds as \Pds[1].
The \W{P}-containedness follows from \cref{thm:wp contained ntm}.
A non-deterministic Turing machine can guess a set of vertices in $k \log \abs{V}$ time and check whether it is an $l$-power dominating set in polynomial time.

We further show that $l$-\Pds is \W{P}-hard if $l \geq 1$ by reduction from \Pds.
\begin{proof}
  Let $G=(V,E)$ be an instance of \Pds.
  We construct a graph $G'=(V \cup V_1, E \cup E_1)$ by attaching $l - 1$ new degree-one vertices to each vertex.

  Let $S$ be a power dominating set of $G$ of size $k$.
  We show that $S$ is an $l$-power dominating set of $G'$.
  The vertices in $N[S]$ are observed by the domination rule.
  If during the application of the propagation rule an observed vertex $v \in V$ has precisely one unobserved neighbor, its counterpart in $G'$ has precisely $l$ unobserved neighbors.
  Hence $S$ is an $l$-power dominating set of $G'$.

  Now let $S*$ be an $l$-power dominating set of $G'$ with $\abs{S*} = k$.
  We construct $S = S* \setminus V_1 \cup \set{v \in V \mid N(v) \cap V_1 \cap S \neq \emptyset}$ by replacing all vertices in $S \cap V_1$ with their neighbor.
  Clearly $\abs{S} \leq \abs{S*}$, because for every vertex we newly insert, we remove at least one other vertex.
  Because the vertices in $V_1$ can each only observe their single neighbor, if $S*$ is an $l$-power dominating set, so is $S$.
  $S$ is also a power dominating set of $G$.
  If during the application of the $l$-propagation rule a vertex in $G'$ has at most $l$ unobserved neighbors, its counterpart in $G$ has at most one unobserved neighbor by construction and thus the regular propagation rule applies in $G$.
  \todo{Extend to k as input with booster vertex if k > deg(v)}
\end{proof}

==> sections/wpcomplete.tex <==
\section{\PDS is \W{P} complete}
In this section we show that \PDS is \W{P} complete.
We show this by introducing an auxiliary problem which we call \IPDS and the using a circular reduction \WMCS $\leftarrow$ \PDS $\leftrightarrow$ \IPDS $\leftarrow$ \WMCS.

\subsection{\PDS is in \W{P}}
The containedness of \PDS in \W{P} has been shown by \citeauthor{kneis2006parameterized}\parencite{kneis2006parameterized}.
They used a result by \citeauthor{cai1995structure}\parencite{cai1995structure}
\begin{proposition}[{\citeauthor{cai1995structure}\cite[][Thm. 3.7]{cai1995structure}}, formulation due to \cite{kneis2006parameterized}]
	\todo{Is the reformulation by \cite{kneis2006parameterized} actually correct (it works for \Pds, but does it always work)?}
	Let $L$ be a parameterized problem in \NP.
	Then $L \in \W{P}$ if and only if there is a non-deterministic Turing machine $M$ deciding $L$, such that given an input $<x, k> \in L$, $M$ performs at most $f(k) \log \abs{x}$ non-deterministic steps and $p(\abs{x} + k)$ deterministic steps.
	\label{lem:wp contained ntm}
\end{proposition}

\begin{proof}[\citeauthor{kneis2006parameterized}]
	A nondeterministic Turing machine can guess a power dominating set $S$ in $k \log \abs{V}$ nondeterministic steps.
	It can then check whether all vertices in $G$ are observed by $S$ in polynomial time.
\end{proof}

We provide a longer, but more tangible alternative proof.%, that relies on the \W{P} completeness of \WMCS which was shown in \cite{abrahamson1995fixed}.
Our proof relies on a reduction of \Pds to \Wmcs which is \W{P} complete and thus in \W{P}.

\begin{proof}
	Given an instance $G = (V, E)$ and parameter $k$, we construct a weighted monotone circuit $C$ with the same parameter $k$.
	Our circuit consists of alternating layers of \AND- and \OR-gates.
	Each layer of \OR-gates in this circuit models the observation status after another application of the propagation rule.

	We construct $C$ as follows.
	In the input layer $\Vin$ we have one node for each $v \in V$.
	Next we add a layer $\Vor^{(1)}$ of $\abs{V}$ \OR-gates, again one for every $v \in V$.
	We add an edge from $v_x \in \Vin$ to $v_y \in \Vor^{(1)}$ if and only if $xy \in E$.
	After this first layer we add $2\abs{V}$ alternating layers of \AND- and \OR-gates.
	For $i \in \set{1,\dots,\abs{V}}$ we use the following construction.
	A vertex is observed in step $i$ if it was observed before or if one of its observed neighbors has only one unobserved neighbor.
	For each vertex $x \in V$ we thus insert one new \AND-gate $w_{x,x}$ only connected to $v_x^{(i)} \in \Vor^{(i)}$ and one new \AND-gate $w_{x,y}$ for every neighbor $y \in N(x)$.
	For all transitive neighbors $z \in N[y] \setminus \set{x}$ we add an edge $w_{x,y} v_z^{(i)}$.
	The following layer of \OR-gates $\Vor^{(i+1)}$ again has one gate for each $x \in V$.
	For each given $x \in V$, the gate $v_x^{(i+1)} \in \Vor^{(i+1)}$ connects to all $w_{x,y} \in \Vand^{(i)}$.
	Finally we add a single \AND-gate collecting the results of all \OR gates in $\Vor^{(\abs{V}+1)}$ and connect it to the output of the circuit.
	This construction clearly runs in polynomial time and creates a circuit with $\bigO(\abs{V}^2)$ \OR-gates and $\bigO(\abs{V}\abs{E})$ \AND-gates.

	The correctness follows from the construction by iterative application of the propagation rule.
	By construction, each gate $v_x^{(1)}$ in $\Vor^{(1)}$ output true if and only if $x \in V$ is dominated by the domination rule.
	In all other layers $\Vor^{(i+1)}$ each $v_x^{(i+1)}$ output true if and only if either $v_x^{(i)}$ was already true or $x$ is observed by one of its neighbors through the propagation rule.
\end{proof}\todoi{Better proof, picture}

\subsection{\IPDS}
\newcommand{\Eu}{\overbar{E}}
\newcommand{\Ed}{\vec{E}}
\IPDS(\Ipds) is a modification of \PDS that operates on semi-directed graphs.\todo{better name? „implicating“ sounds a bit like „accusing“}
Before we define \IPDS, we introduce some more notation.
Let $G=(V, \Eu\cup\Ed)$ be a semi-directed graph with a set of undirected edges $\Eu$ and a set of directed edges $\Ed \subseteq V^2$ such that $\Eu \cap \Ed = \emptyset$.
We define the \emph{neighborhood} $N(v)$ of a vertex $v \in V$ to only include neighbors reached via an undirected edge: $N(v) = \set[]{w \in V \mid vw \in \Eu}$.
The \emph{closed neighborhood} $N[v] = \set{v} \cup N(v)$ also includes the vertex itself.

Like \PDS, \IPDS is also based on a set of rules.
The domination and propagation rules for \Ipds are the same as for \Pds and consider only undirected edges.
The \emph{domination rule} for \Ipds, like the one for \Pds, states that a vertex $v \in S$ observes itself and all its neighbors, i.e. $v \in S \implies N[v] \text{ observed}$.
We restrict the \emph{propagation rule} to undirected edges, i.e. if a vertex $v$ is observed and $w$ is the only unobserved vertex in $N(v)$, then $w$ is also observed.
\Ipds uses an additional \emph{implication rule}.
If for any directed edge $(v, w) \in \Ed$ the first vertex $v$ is observed, $w$ becomes observed, too.
Because of this rule, we refer to the directed edges as \emph{implication edges}.
Note that implication edges don't affect the domination and propagation rules and interact only via the implication rule.

\IPDS is then defined as the problem of finding a set $S$ of size at most $k$ that observes a given semidirected graph $G = (V, \Eu \cup \Ed)$ after application of the domination rule and exhaustive application of the modified propagation rule and the implication rule.
If the input does not contain any implication edges, this is the same as \PDS.

First, we show that \IPDS can be reduced to \PDS, increasing the parameter $k$ to $k+1$.
We use the following two gadgets to represent the implication edges with undirected edges and additional vertices.

To construct a gadget for the implication edge we first construct a helper gadget.
Implication edges allow propagation of the observation status to more than one neighbor.
We thus need a way to propagate observation to more than one vertex using only the domination and propagation rules.
Our solution is the gadget depicted in \Cref{fig:booster full}.
This gadget consist two parts, one in the boosted edge and a globally unique path $B$.
The path $B$ is a $P_3$ with central vertex $b$.
To boost\todo{Find a better formulation for the boosted edge} an edge $xy$ we insert a node $v$ into $xy$ and add an edge $vb$.
We call the resulting path $xvy$ a \emph{boosted edge} and refer to it only by its endpoints as $xy$.

\begin{figure}
	\subcaptionbox{Booster edge shorthand\label{fig:booster short}}[.48\linewidth]{\input{figures/booster/short}}
	\subcaptionbox{Implication edge shorthand\label{fig:implication short}}[.48\linewidth]{\input{figures/implication/short}}
	\newline
	\subcaptionbox{Expanded booster gadget\label{fig:booster full}}[.48\linewidth]{\input{figures/booster/expanded}}
	\subcaptionbox{Expanded implication gadget\label{fig:implication full}}[.48\linewidth]{\input{figures/implication/expanded}}
	\caption{Gadgets and shorthand notations\todoin{more detailed description}}
\end{figure}

\begin{lemma}
	\label{lem:booster}
	Be $b$ be in the power dominating set and let $xy$ be a boosted edge.
	Then, if one endpoint $x$ is observed the other endpoint $y$ becomes observed, too.
	\begin{proof}
		This follows directly from the domination and propagation rules.
		The central node $v$ of the boosted edge is dominated by $b$.
		If either $x$ or $y$ is dominated, the other vertex is the only undominated neighbor of $v$ and it thus becomes observed by the propagation rule.
		%Any valid power dominating set must contain at least one vertex in $B$.
		%This is easy to see if we assume that $B\cap S = \emptyset$.
		%Then $b$ has two unobserved neighbors which must remain unobserved because the propagation rule cannot be applied to $b$.
		%
		%Selecting $b$ over one of the other two vertices never increases the size of a power dominating set.
		%We can thus safely assume that $b$ is selected in a minimal power dominating set and all its neighbors to be observed by the domination rule.
		%
		%For a similar reason there exists a minimum power dominating set $S$ which does not contain $v$.
		%If $v$ is in the power dominating set, we can always select $x$ instead.
		%Now let $x$ be observed.
		%As $x$ is the only unobserved neighbor of $v$, which is in turn observed by $b$, we can apply the propagation rule to $v$ and observe $y$.
	\end{proof}
\end{lemma}

We use the booster edge to construct the full gadget for the implication edges.
The construction is depicted in \Cref{fig:implication full}.
This second gadget has to ensure that domination is only propagated in one direction.
Let $e =(x,y) \in \Ed$ be an implication edge.
We denote by $I_e$ the set of inner vertices of the gadget, i.e. $x$, $y$ and the booster path are not part of $I_e$.

Let $G = (V, \Eu \cup \Ed)$ be a semi-directed graph and let $G' = (V', E')$ be the result of replacing all implication edges with the gadget in \Cref{fig:implication full}.
Then $G$ has an implicating power dominating set $S \subseteq V$ of size $k$ if and only if $G'$ has a power dominating set $S' \subseteq V'$ of size $k + 1$.\todo{restrict $k < \abs{V}?$}

\begin{proof}
	Note that the claim is trivially true, if $\Ed = \emptyset$.
	In this case $G' = (V \cup V(B), \Eu \cup E(B))$ and thus $S' = S \cup {b}$ where $b$ can be any vertex in the booster path $B$.

	First we observe that $S'$ must contain at least one vertex in the booster path $B$.
	If $B \ cap S = \emptyset$, $b$ always has two unobserved neighbors and the propagation rule can thus not be applied leaving the unobserved.
	
	We show that $S' = S \cup \set[]{b}$ is a power dominating set of $G'$ if $S$ is an implicating power dominating set of $G$.
	For this, it suffices to show that the implication edge gadget simulates the implication rule and that the propagation rule is unaffected by the gadget.
	Let $x$ be observed.
	Then by applying of \Cref{lem:booster} and the propagation rule $y$ and all vertices in the gadget become observed, too.
	The domination rule is unaffected by the gadget, i.e. vertices that were dominated by the domination rule in $G$ are dominated by the domination rule in $G'$.
	The gadget adds additional neighbors to both $x$ and $y$ which could impact the application of the propagation rule.
	These neighbors are, however, dominated by $b$ and thus if $x$ or $y$ could propagate their observation status in $G$, they can also do so in $G'$.
	Thus, $S'$ is a power dominating set of $G'$ with size $\abs{S'} = \abs{S} + 1$.
	
	Next we show that if $S'$ is a power dominating set of $G'$, there exists an implicating power dominating set $S$ of $G$ of size $\abs{S'} = \abs{S} + 1$.
	%Assume in the following that $S'$ is a power dominating set of minimum size.
	If for any $e = (x,y) \in \Ed$ the booster gadget $I_e \cap S \neq \emptyset$ we construct a new set $S'' = S' \setminus (I_e \cup B) \cup \set{x,b}$.
	Clearly, $\abs{S''} \leq \abs{S'}$, because $B \cap S \neq \emptyset$ and $I_e \cap S \neq \emptyset$.
	By applying the domination rule and propagation rule iteratively, all vertices in $I_e$ and $y$ become observed by $S''$.
	%Thus, if $S'$ is a minimum power dominating set of $G'$, so is $S''$.
	We apply this to all implication edges $e \in Ed$ and obtain the power dominating set $S''$ of $G'$.
	Note that $\abs{S''} \leq \abs{S'}$.
	
	As a last step we show that $S = S'' \setminus B$ is an implicating power dominating set of $G$.
	From the same argument as above, we know that if $x$ is observed $y$ is also observed in $G'$ and it is observed by the implication rule in $G$.
	It remains to show that observation does not propagate from $y$ to $x$ through $I_e$.
	Assume $y$ is observed and $x$ is unobserved.
	Then by \Cref{lem:booster} $y$'s neighbor $c$ is also observed.
	However, $c$ has two unobserved vertices and thus the propagation rule cannot be applied.
	As long as $x$ remains unobserved, the other non-booster vertices in $I_e$ thus remain unobserved.
	Hence, $S$ is an implicating power dominating set of $G$ and $\abs{S} = \abs{S''\setminus B} = \abs{S'} - 1$ with size $\abs{S} \leq \abs{S'} + 1$.
	
%	First, we show that $b \in S'$ if $\Ed \neq \emptyset$.
	
%	Assume $b \notin S'$.
%	Let $E=(x,y) \in \Ed$  be an implication edge and denote by $I_e$ the vertices added by the implication gadget but not the booster path.
%	Now consider $S'' = S' \setminus (I_e \cup B) \cup \set{b, x}$.
%	If $S'$ is a power dominating set of $G'$, so is $S''$.
%	As $S'$ is of minimum size and because $B \cap S' \neq \emptyset$, we know that $\abs{S'} \leq \abs{S''} \leq \abs{S'} + 1$.
%	Thus $\abs{S \cap I_e} \leq 1$.
%	Because $b \notin S$, the domination and propagation rule cannot observe $I_e$.
%	Hence we conclude that $b \in S$.
\end{proof}

\begin{corollary}
	\IPDS and \PDS have the same parametric complexity with respect to their natural parameterization.
\end{corollary}

\subsection{Representing WMNS as \PDS}

It remains to show that \IPDS is \W{P}-hard.
Let $C=(\Vin \cup \Vand \cup \Vor \cup \set{\text{out}},E)$ be a weighted monotone circuit.
We use the gadget in \Cref{fig:and gadget} to represent \AND-gates and we add all directed edges $\set{(\text{out},w)\mid w \in \Vin}$.
With this gadget we already obtain a valid power dominating set from a satisfying assignment.
But we also have to ensure that a minimum power dominating set containing only input vertices exists.

\begin{figure}
	\subcaptionbox{Input monotone circuit\label{fig:monotone circuit}}[.27\linewidth]{\input{figures/reduction/circuit}}
	\subcaptionbox{Corresponding \Ipds instance. For better readibility the circuit is only shown once and the booster path is left out.\label{fig:ipds circuit} }[.53\linewidth]{\input{figures/reduction/pds}}
	\subcaptionbox{\AND-Gadget\label{fig:and gadget}}[.19\linewidth]{\input{figures/reduction/and}}
	\caption{Example of a transformation from a circuit to an \Ipds instance\todoin{More detailed description}}
\end{figure}

We construct $G$ as the disjoint union of $\abs{\Vin} + 1$ copies $C^{(j)}$ of $C$ using the gadget in \Cref{fig:and gadget}.
Then we add a clique $X=\set[]{x_1,\dots,x_{\abs{\Vin}+1}}$ of size $\abs{\Vin}$ and add edges from $x_i$ to each corresponding input vertex in the copied circuits $\Vin^{(j)}$.
An example of this transformation is depicted in \Cref{fig:monotone circuit} and \Cref{fig:ipds circuit}.

We show that $C$ has a satisfying assignment of weight $k$ if and only if $G$ has an implicating power dominating set of size $k$.
\begin{proof}
	Let $A$ be a satisfying assignment of weight $k$.
	Then we find an implicating power dominating set $S$ by using the $x_i$ corresponding to the true inputs in $A$.
	By our construction the \OR-gates are observed by the implication rule if any of their input vertices are observed.
	And gates, represented by our gadget, are observed, if and only if all of their input vertices are observed.
	If an input vertex is observed, it observes its auxiliary vertex on the input edge by the implication rule.
	The auxiliary vertex, in turn, observes the central vertex by the propagation rule.
	The central vertex observes the output vertex of the gadget by the propagation rule if and only if all input vertices are observed.
	This means that observation propagates through each copied circuit $C^{(j)}$ the same way as truth-values of the assignment do.
	Hence $S$ observes $\text{out}^{(j)}$ at some point and in turn the whole copied circuit $C^{(j)}$ via the implication edges from $\text{out}^{(j)}$ to the copied inputs.
	
	If $k \geq \abs{\Vin}$ we can find a trivial satisfying assignment $A = \Vin$.
	Thus assume that $k < \abs{\Vin}$.
	Let $S$ be an implicating power dominating set of $G$ with size $\abs{S} = k$.
	We show that $X \cap S$ is also a power dominating set.
	As $k < \abs{\Vin}$ there are at least two copies $C^{(j)}$ and $C^{(l)}$  without any vertices in $S$.
	Hence, all vertices in $X$ have at least two unobserved neighbors and cannot propagate their observation status.
	Because $S$ is an implicating power dominating set, both $C^{(j)}$ and $C^{(l)}$ are observed by $S$.
	We ruled out the propagation rule, so these copies must be observed by the domination rule from vertices in $X \cap S$.
	All copies are identical and thus $X \cap S$ is an implicating power dominating set of $G$ of size at most $k$.
	
	\IPDS is thus \W{P}-hard.
\end{proof}

\begin{corollary}
	\PDS is \W{P} complete.
\end{corollary}

% random observation that also follows
The construciton we used in the proof to constrain $S$ to a subset $X \subseteq V$ directly leads us to another interesting conclusion.
It does not depend on the underlying graph being a circuit and does not require any directed edges.
\PDS is thus also \W{P}-complete if the power dominating set is constrained to a subset of the vertices, where this subset is an additional input.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> solving.tex <==
%! Tex root = ../paper.tex
\section{Solving \PDS}
\label{sec:solving}

In this section, we give an algorithm for solving \extension{\Pds}.
Our algorithm consists of different phases.
In the first phase, we apply the reduction rules described in \cref{sec:reduction rules}.
Each rule either shrinks the graph or decides for a vertex that it should be pre-selected or excluded.
We prove that the rules are safe, i.e., they yield equivalent instances.
Afterwards, in \cref{sec:sub-problems} we split the instance into several components that can be solved independently.
Finally, each of these subinstances is solved exactly using the implicit hitting set approach~\cite{bozeman2018RestrictedPD} with our improved strategy for finding new sets that need to be hit; see Section~\ref{sec:kernel solver}.

We note that these phases are somewhat modular in the sense that one could easily add further reduction rules or that one can replace the algorithm for solving the kernel in the final step.
In our experiments in Section~\ref{sec:experiments}, we also use an MILP for this step.
This MILP formulation is based on the formulation for \Pds by Jovanovic and Voss~\cite{jovanovic2020fixed} and we discuss our adjustments in \cref{sec:milp formulation}.
Moreover, instead of solving the subinstances optimally, one can instead use a heuristic solver.
In the latter case, the preceding application of our reduction rules and splitting into subinstances then helps to find better solutions rather than improving the running time of exact solvers.
This is used in our experiments to find upper bounds on the power domination number before we have an exact solution.

\subsection{Reduction Rules}
\label{sec:reduction rules}

\makeatletter
\newcommand{\reductionname}[1]{% \settheoremtag{<tag>}
  \let\oldthereduction\thereduction% Store \thetheorem
  \renewcommand{\thereduction}{\texttt{#1}}% Redefine it to a fixed value
  \g@addto@macro\endreduction{% At \end{reduction}, ...
  %\addtocounter{theorem}{-1}% ...restore theorem counter value and...
  \global\let\thereduction\oldthereduction}% ...restore \thetheorem
}
\makeatother
%\newcommand{\reduction}[1]{\textsc{\pgfkeysvalueof{/pds/rule/#1}}}

Many of our reduction rules are local in the sense that they transform one substructure into a different substructure.
Most of our local reduction rules are illustrated in \Cref{fig:local-red-rules}.
%In the following, we specify additional reduction rules that are either non-local or otherwise difficult to illustrate.
For proofs of safeness, see \Cref{sec:reduct-rules-appendix}.

\begin{figure}
  \begin{subcaptionblock}{\linewidth}
    \centering
    \input{figures/rules/leaf1.tikz}
    \caption{\ref{red:leaf 1}: If an undecided leaf is attached to a non-excluded vertex. The reduction rule excludes the leaf.\label{fig:red:leaf 1}}
  \end{subcaptionblock}
  \begin{subcaptionblock}{\linewidth}
    \centering
    \input{figures/rules/leaf21.tikz}
    \hspace{2cm}
    \input{figures/rules/leaf22.tikz}
    \caption{\ref{red:leaf 2}: Two cases of excluded leaves attached to a vertex. On the left, the parent vertex is propagating and becomes non-propagating. On the right, the parent vertex is non-propagating and becomes pre-selected. The attached leaf is removed in both cases.\label{fig:red:leaf 2}}
  \end{subcaptionblock}
  \begin{subcaptionblock}{\linewidth}
    \centering
    \input{figures/rules/path1.tikz}
    \caption{\ref{red:path 1}: A vertex $v$ of degree two can safely be excluded if it has an undecided neighbor. \label{fig:red:path 1}}
  \end{subcaptionblock}
  \begin{subcaptionblock}{\linewidth}
    \centering
    \input{figures/rules/path2.tikz}
    \caption{\ref{red:path 2}: The neighbors $x$ and $v$ of degree two can be merged if $x$ is not adjacent to $v$'s other neighbor~$y$. \label{fig:red:path 2}}
  \end{subcaptionblock}
  \begin{subcaptionblock}{\linewidth}
    \centering
    \input{figures/rules/path4.tikz}
    \caption{\ref{red:path 3}: If $v$ is observed and has two non-adjacent unobserved neighbors of degree two, $x$ and $y$, with $y$ being excluded, then we remove $y$ and the edge $xv$ and connect $x$ to the other neighbor  $z$ of $y$.\label{fig:red:path 3}}
  \end{subcaptionblock}
  \begin{subcaptionblock}{\linewidth}
    \centering
    \input{figures/rules/path3.tikz}
    \caption{\ref{red:tri}: We pre-select the undecided and remove the two vertices of degree two in the triangle.\label{fig:red tri}}
  \end{subcaptionblock}
  \begin{subcaptionblock}{\linewidth}
    \centering
    \input{figures/rules/path5.tikz}
    \caption{\ref{red:path 5}: If an excluded vertex is surrounded by non-propagating vertices, only one of which is not excluded, we pre-select the non-excluded vertex.\label{fig:red:path 5}}
  \end{subcaptionblock}
  \caption{Illustrated overview of the local reduction rules. Round vertices {\tikz[pds instance] \node[node,propagating] {};} are propagating, triangular vertices {\tikz[pds instance] \node[node,propagating=no] {};} are non-propagating, square vertices \tikz[pds instance] \node[node] {}; may be propagating or non-propagating. Hollow vertices {\tikz[pds instance] \node[node,solution=no] {};} are excluded from a solution, vertices filled black {\tikz[pds instance] \node[node,solution=undecided] {};} are undecided, red vertices {\tikz[pds instance] \node[node,solution=yes,propagating=no] {};} are pre-selected. Vertices filled gray {\tikz[pds instance] \node[node,solution=dontcare] {};} may be undecided, excluded or pre-selected. Green vertices {\tikz[pds instance] \node[node,observed,solution=no] {};} are observed but not pre-selected. The non-existence of an edge is indicated in red {\tikz[pds instance] \draw[nonedge] (0,0) -- ++(0.5,0);}.}
  \label{fig:local-red-rules}
\end{figure}


Our first set of reduction rules stems from the observation that leaves, i.e. vertices of degree one, are usually not part of an optimum solution.
To keep the rules safe, we only delete excluded leaves and only exclude leaves that can be observed from some other vertex.
See \cref{fig:red:leaf 1,fig:red:leaf 2} for a visual example.

\reductionname{Deg1a}
\begin{reduction}[restate=reductionDegIa]
  \label{red:leaf 1}
  Let $v$ be an undecided leaf attached to a non-excluded vertex $w$.
  Then mark $v$ as excluded.
\end{reduction}

\reductionname{Deg1b}
\begin{reduction}[restate=reductionDegIb]
  \label{red:leaf 2}
  Let $v$ be an excluded leaf attached to $w$.
  If $w$ is propagating, delete $v$ and set $w$ to non-propagating.
  If $w$ is not excluded and not propagating, delete $v$ and select $w$, i.e., set $X \gets X \cup \set{w}$.
\end{reduction}

A case very similar to \ref{red:leaf 2} is illustrated in \cref{fig:red tri}.
Two adjacent vertices $x$ and $y$ of degree two share an undecided neighbor $z$
Similar to \cref{lem:booster vertex}, we can always select $z$.

\reductionname{Tri} %todo: rename → Tri rule
\begin{reduction}[restate=reductionTri]
  \label{red:tri}
  Let $x$ and $y$ be two adjacent vertices of degree two with a common neighbor $z$.
  If $z$ is undecided, select $z$ and delete $x$ and $y$.
\end{reduction}

The possibility of applying the propagation rule leads to a number of further reduction rules related two vertices of degree two, illustrated in \cref{fig:red:path 1,fig:red:path 2,fig:red:path 3}.
Note, for example, that vertices of degree two with an undecided neighbor never need to be selected.
One can always select the neighbor instead.

\reductionname{Deg2a}
\begin{reduction}[restate=reductionDegIIa]
  \label{red:path 1}
  Let $v \in Z \setminus (X \cup Y)$ be an undecided propagating vertex with $d(v) = 2$ and let $x$ and $y$ be its neighbors.
  If $x$ and $y$ are not adjacent and if at least one of $x$ and $y$ is not excluded, exclude $v$.
\end{reduction}

If two adjacent vertices have degree two, the propagation rule ensures that if one becomes observed, the other becomes observed, too.
The two vertices can thus be merged.

\reductionname{Deg2b}
\begin{reduction}[restate=reductionDegIIb]
  \label{red:path 2}
  Let $v \in Y \cap Z$ be an excluded propagating vertex with $d(v) = 2$ and let $x$ and $y$ be its neighbors.
  If $x$ and $y$ are not adjacent and if at least one of $x$ and $y$ is propagating and has degree 2, delete $v$ and add an edge between $x$ and $y$ instead.
\end{reduction}

Something similar happens when two unobserved vertices of degree two share an observed neighbor with no other unobserved neighbors.
Recall the gadget used in the removal of the booster edges in \cref{lem:booster gadget}, which works in the same way.
If one of the two unobserved vertices becomes observed, the other becomes observed by the propagation rule.
If both vertices additionally have degree two, they thus behave like a single vertex to their other two neighbors.

\reductionname{Deg2c}
\begin{reduction}[restate=reductionDegIIc]
  \label{red:path 3}
  Let $v$ be an observed excluded propagating vertex with precisely two unobserved neighbors, both of degree two, $x$ and $y$.
  If $x$ and $y$ are not connected, $y$ must have another neighbor $z$.
  In this case remove $y$ and the edge $xv$ and add a new edge $xz$.
\end{reduction}

There are several trivial cases where a vertex must be selected to form a feasible solution.
If an undecided unobserved vertex has no neighbors, clearly that vertex must be selected.
See \cref{fig:red:path 5} for an example.
Similarly, if an unobserved excluded vertex has only non-propagating only one of which is not excluded, that neighbor must be selected.

\reductionname{OnlyN} %todo: rename?
\begin{reduction}[restate=reductionOnlyN]
  \label{red:path 5}
  Let $v$ be an excluded propagating vertex of degree two with two non-propagating neighbors $x$ and $y$.
  If $x$ is excluded and $y$ is undecided, select $y$.
\end{reduction}

\reductionname{Isol}
\begin{reduction}[name=Isolated,restate=reductionIsol]
  \label{red:isolated}
  Let $v$ be an undecided isolated vertex.
  Then pre-select $v$.
\end{reduction}

\reductionname{ObsNP}
\begin{reduction}[name=Observed Non-Propagating,restate=reductionObsNP]
  \label{red:observed non-zi}
  Let $v$ be an observed, non-propagating and excluded vertex.
  Then delete $v$.
\end{reduction}
%
We do not need the propagation rule to observe the vertices observed by the currently selected vertices.
Instead we can connect all those vertices directly to selected vertices and observe them by the domination rule instead and remove the now redundant edges.
This rule is most useful when combined with the other rules.
In particular, all vertices with only observed neighbors become leaves and are then removed by \cref{red:leaf 1,red:leaf 2}.

\reductionname{ObsE}
\begin{reduction}[name=Observed Edge,restate=reductionObsE]
  \label{red:observed edge}
  Let $vw \in E$ be an edge with two observed but not pre-selected endpoints and let $x \in X$.
  Then delete $vw$ and instead insert edges $vx$ and $wx$.
\end{reduction}

The previous rules identified vertices to be forbidden from a solution by looking at small localized structures.
We can identify those vertices and many more by looking at the vertices that would become observed by selecting a vertex.
For the next two reduction rules, we introduce the concept of \emph{observation neighborhood}.
For a set of vertices $U \subseteq V$ the observation neighborhood is the set of vertices that is observed when selecting $U$ in addition to all pre-selected vertices and applying the observation rules exhaustively.
For convenience, we define the observation neighborhood of a single vertex $v$ to be the observation neighborhood of the single element set $\set{v}$.
We use the observation neighborhood to formulate the following reduction rule.

\reductionname{Dom}
\begin{reduction}[name=Domination,restate=reductionDom]
  \label{red:domination}
  If the closed neighborhood of some undecided vertex $w$ is contained in the observation neighborhood of some other undecided vertex $v$, exclude $w$.
\end{reduction}

\Cref{red:leaf 2,red:tri,red:path 5} can be seen as special cases of a more general rule.
All three identify vertices that must be active in a minimum solution.
There are, however some vertices that must be active in every solution.
We can identify all those vertices by looking at the observation neighborhood of all other undecided vertices.
This tells us if there is a solution in which the vertex is not selected.

\reductionname{NecN}
\begin{reduction}[name=Necessary Node,restate=reductionNecN]
  \label{red:necessary}
  Let $v \in B$ be an undecided vertex.
  If the observation neighborhood of all undecided vertices except $v$ does not contain all vertices in $G$, select $v$.
\end{reduction}

We note that Binkele-Raible and Fernau~\cite{binkele2012exact} already introduced reduction rules for their exponential-time algorithm.
We do not use them in our algorithm as they are not generally applicable but rather require a specific situation.
The only exception \cite[``isolated'']{binkele2012exact} that is applicable is superseded by a combination of our reduction rules.

% \paragraph{Other rules}

% Prior work by Binkele-Raible and Fernau~\cite{binkele2012exact} introduced reduction rules for \textsc{simple-\Pds} which only worked under specific assumptions and in a particular order.
% Our rules differ in that each of them is safe on its own, i.e. every rule produces an equivalent instance in terms of feasibility and optimality.
% This allows combining the rules freely in any order.
% Additionally, we leverage the non-propagating vertices, leading to new reduction rules.

% The following reduction rules for \extension{\textsc{simple-\Pds}} were used by Binkele-Raible and Fernau~\cite{binkele2012exact}.

% \reductionname{FullObs}
% \begin{reduction}[Fully Observed („Isolated“ in \cite{binkele2012exact})]
%   \label{red:fully observed}
%   Let $v \in B$ be an undecided vertex.
%   If $N[v]$ is observed, exclude $v$.
% \end{reduction}

% We do not include this rule in our reduction because all vertices to which it applies are removed by successively applying \cref{red:observed edge,red:leaf 2}.
% Such vertices would also be excluded by \cref{red:domination}.
% The other rules proposed by Binkele-Raible and Fernau are not applicable to general \extension{\Pds} and only work in conjunction with their branching algorithm on \Pds-instances.
% \todo{Elaborate argument?}

\subsubsection{Order of Application}
\label{sec:order application}

In a first step, use a depth first search and process the vertices in post-order to apply the rules \labelcref{red:leaf 1,red:leaf 2,red:path 1}.
The order in which we process the vertices is important here, as it makes sure that attached paths are properly reduced.
This is only relevant for this first application of the reduction rules and in later applications, we process the vertices and edges in arbitrary order.
After this initial application, we iterate the following three steps until no reduction rules can be applied.
(i) Iterate the application of the local reduction rules (\ref{red:leaf 1}, \ref{red:leaf 2}, \ref{red:path 1}, \ref{red:path 2}, \ref{red:tri}, \ref{red:path 3}, \ref{red:path 5}, \ref{red:observed non-zi}, \ref{red:observed edge}) until no local reduction rule is applicable.
(ii) Apply the non-local rule \ref{red:domination}.
(iii) Apply the non-local rule \ref{red:necessary}.

We note that applying \ref{red:domination} once to all vertices is exhaustive in the sense that it cannot be applied again immediately afterwards.
It can, however, become applicable again after rerunning the other reduction rules.
The same is true for \ref{red:necessary}.

Our reasoning for this sequence of application is that the local rules are more efficient than the non-local once.
Thus, we first apply the cheap rules exhaustively before resorting to the expensive ones.
Preliminary experiments showed that further tweaking the order of application has only minor effect on the kernel size and run time.

\subsubsection{Implementation Notes}

The naïve implementation of the reduction rules can be very slow, in particular for the non-local rules.
The costly operation in those rules is the computation of the observation neighborhood.
We thus use a specialized data structure that allows us to pre-select and deselect vertices in arbitrary order.
Each time we pre-select a vertex, we also update the observed vertices and keep track of which vertex propagates to which other vertex.
For de-selecting vertices, we only mark vertices as unobserved, that were directly or indirectly observed by the deselected vertex.
Being able to select and deselect arbitrary vertices allows a straightforward implementation of the non-local rules.
%In \cref{red:domination} we select a vertex and check for all vertices that become observed and their neighbors whether they have any unobserved neighbors left.
%Afterwards we deselect that vertex again.
%Similarly for \cref{red:necessary}, we select all vertices and deselect each undecided vertex in turn to see whether any unobserved vertices remain.

\subsection{Split into Subinstances}
\label{sec:sub-problems}

\begin{figure}
  \input{figures/reduction/subproblems.tikz}
  \caption{Example of independent sub-problems arising from the kernel on the left. Each connected component on the right can be solved independent from the others.}
  \label{fig:red:sub problems}
\end{figure}

While the propagation rule may have non-local effects within the whole graph, propagation cannot pass through selected vertices.
This is formalized by the following theorem.

\begin{restatable}{theorem}{splitIntoSubinstances}
  Let $G = (V, E)$ be the graph with pre-selected vertices $X \subseteq V$ and let $C_1,\dots,C_\ell \subseteq V$ be the vertices in the connected components of the sub-graph of $G$ induced by $V \setminus X$.
  Further let $S_1,\dots,S_\ell$ be minimum power dominating sets of the subgraphs induced by $N[C_1],\dots,N[C_\ell]$.
  Then $S = S_1 \cup \dots \cup S_\ell$ is a minimum power dominating set of $G$.
\end{restatable}

These sub-problems can be identified in linear time using a depth-first search restarting at unexplored non-active nodes while ignoring outgoing edges of active nodes.
See \cref{fig:red:sub problems} for an example of an instance split into subinstances.

\subsection{Solving the Kernel Via Implicit Hitting Set}
\label{sec:kernel solver}

We briefly describe the implicit hitting set approach.
Compared to how Bozeman et al.~\cite{bozeman2018RestrictedPD} introduced it, we allow non-propagating vertices.
However, this does not change any of the proofs and thus the approach directly translates to this slightly more general setting.

In a graph $G$, a \emph{fort} is a non-empty subset of vertices $F \subseteq V(G)$ such that no propagating vertex outside $F$ is adjacent to precisely one vertex in $F$.
A power dominating set must be a hitting set of the family of all \emph{fort neighborhoods} in $G$, i.e., if $F$ is a fort and $S$ is a power dominating set, then $N[F] \cap S \neq \emptyset$.
Conversely, if a hitting set for a family $\mathcal F$ of fort neighborhoods is not a power dominating set, then one can find an additional fort of $G$ whose neighborhood is not in $\mathcal F$.

This yields the following algorithm.
Start with some set $\mathcal F$ of fort neighborhoods.
Compute a minimum hitting set $H$ for $\mathcal F$.
If $H$ is already a power dominating set, we have found the optimum.
Otherwise, we construct at least one new fort neighborhood and add it to $\mathcal F$.

One core ingredient of this approach is the choice of which fort neighborhoods to add to~$\mathcal F$.
Previous approaches~\cite{smith2020OptimalSP,bozeman2018RestrictedPD} aimed at finding forts or fort neighborhoods that are as small as possible.
The reasoning behind this is that the set of all fort neighborhoods can be exponentially large (even when restricted to those that are minimal with respect to inclusion) and thus it makes sense to add sets that are as restrictive as possible, hoping that only few sets suffice before the \HS solution yields a \Pds solution.
However, finding forts of minimum size or minimum size fort neighborhoods is difficult while just finding any fort is easy.
Moreover, if we add only few forts in every step, we have to potentially solve more \HS instances.
We thus propose to instead find multiple forts at once and to add them all to the \HS instance.
Our method of finding forts is based on the following lemma.

\begin{lemma}
  \label{lem:unobserved fort}
  Let $G = (V, E)$ be a graph and let $S \subseteq V$ be a set of selected vertices.
  Let further be $R$ the set of vertices observed by exhaustive application of the observation rules with respect to $S$.
  Then the set of unobserved vertices $V \setminus R$ is a fort.
\end{lemma}
\begin{proof}
  Assume $V \setminus R$ is not a fort.
  Then there exists a propagating vertex $v$ in $R$ that is adjacent to precisely one vertex $w$ in $V \setminus R$, i.e., $v$ has precisely one unobserved neighbor $w$.
  This constradicts the exhaustive application of the propagation rule and thus the set of unobserved vertices is a fort.
\end{proof}

By Lemma~\ref{lem:unobserved fort}, whenever we have a candidate solution that does not yet observe all vertices, we obtain a new fort and can add its neighborhood to the \HS instance $\mathcal F$.
For the new forts, we have two objectives.
First, we want the new fort neighborhood to actually provide new restrictions, i.e., it should not be already hit by the minimum hitting set $H$ of $\mathcal F$.
This is achieved by making sure that the candidate solution $S$ is a superset of the hitting set $H$.
Secondly, we want the resulting forts (i.e., the number of unobserved vertices) to be small.
We achieve this heuristically by greedily considering large candidate solutions.

Specifically, we choose candidate solutions as follows.
Recall, that we consider the extension problem, i.e., we have sets $X$ and $Y$ of pre-selected and excluded vertices, respectively.
Moreover, let $H$ be a minimum hitting set of the current set of fort neighborhoods.
Then $V$ is partitioned into the four sets $X$, $Y$, $H$, and $U = V \setminus H \setminus X \setminus Y$.
Each candidate solution $S$ we consider is a superset of $H \cup X$ and a subset of $H \cup X \cup U$.
We randomly order the vertices in $U = \set{u_1, \dots, u_\ell}$ and define a sequence $U_0, \dots, U_\ell \subseteq U$.
We then consider the candidate solutions $S_i = H \cup X \cup U_i$ for $0 \le i \le \ell$.
As we want to consider large candidate solutions, we start with $U_0 = U$, which clearly yields a solution as the instance would be invalid otherwise.
We obtain the subset $U_i$ from $U_{i - 1}$ as follows.
If $S_{i - 1}$ was a solution, i.e., there were no unobserved vertices, then $U_i = U_{i - 1} \setminus \set{u_i}$.
Otherwise, $U_i = U_{i - 1} \cup \set{u_{i - 1}} \setminus \set{u_i}$.
Note that this makes sure that each candidate solution $S_i$ we consider is either a solution or barley not a solution as $S_i \cup \set{u_i}$ is a solution.

This gives us at least one and up to $\ell$ new fort neighborhoods.
These are not directly added to the set $\mathcal F$.
Instead, we first apply a simple local search to make sure that each fort is minimal with respect to inclusion.
To this end, we iteratively re-select vertices from $U$ that had been removed before and check whether this still results in a non-empty fort.

We note that we only add sets to $\mathcal F$.
Thus, we have to solve a sequence of increasing \HS instances as a subroutine.
To improve the performance of this, one can use lower bounds achieved in earlier iterations as lower bounds for later iterations (\HS is monotone with respect to the addition of sets).

% \subsection{A greedy heuristic}

% To find an upper bound on the power domination number of a graph, we propose a very simple greedy heuristic.
% We enumerate the undecided vertices in descending order by their degree.
% If a vertex is unobserved or has an unobserved neighbor, we add that vertex to the list of selected vertices and update the observed vertices.
% We stop when all vertices are observed.
% If a vertex remains unobserved after enumerating all undecided vertices, the instance is infeasible.
% To improve the bound, we greedily deselect all vertices that are not needed for the current set of selected vertices to be a power dominating set.

% This heuristic can be augmented by exhaustively applying our reduction rules in the beginning and each time we select another vertex.


% \todoin{Move minimum size fort to appendix?}


% \todo{Mention performance here or later?}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:

